Learning Collective Dynamics of Multi-Agent Systems using Event-based Vision

This paper proposes a novel problem: vision-based perception to learn and predict the collective dynamics of multi-agent systems, specifically focusing on interaction strength and convergence time. Multi-agent systems are defined as collections of more than ten interacting agents that exhibit complex group behaviors. Unlike prior studies that assume knowledge of agent positions, we focus on deep learning models to directly predict collective dynamics from visual data, captured as frames or events. Due to the lack of relevant datasets, we create a simulated dataset using a state-of-the-art flocking simulator, coupled with a vision-to-event conversion framework. We empirically demonstrate the effectiveness of event-based representation over traditional frame-based methods in predicting these collective behaviors. Based on our analysis, we present event-based vision for Multi-Agent dynamic Prediction (evMAP), a deep learning architecture designed for real-time, accurate understanding of interaction strength and collective behavior emergence in multi-agent systems.

==> tex/3_eventvision.tex <==
\section{Event-based Vision}

\subsection{Unique Challenges for Multi-Agent Dynamic Prediction}

\begin{figure}[tb]
  \centering
   \includegraphics[width=0.95\linewidth]{figures/task_comparison.pdf}
    % \vspace{-0.1in}
   \caption{\textbf{Event data for various tasks;} semantic segmentation~\cite{gehrig2021dsec}, object detection~\cite{de2020large}, depth estimation~\cite{zhu2018multivehicle}, and multi-agent dynamic prediction (this work). Long-term spatiotemporal information becomes more crucial for multi-agent dynamic prediction.}
   \label{fig:task_comparison}
   % \vspace{-0.1in}
\end{figure}


There has been a lot of efforts on utilizing event-based representations for various vision tasks, such as object recognition [ref], semantic segmentation [ref], object detection [ref]. Leveraging temporal or spatiotemporal information enhances perception accuracy, though these tasks can also achieve moderate accuracy using solely spatial information [ref]. For example, analyzing an event-based frame or a brief time span allows for the segmentation of road regions, detection of cars, or depth estimation of different areas (Figure~\ref{fig:task_comparison}). However, predicting agent interactions or collective behavior becomes significantly easier with the observation over extended periods, highlighting the importance of long-term spatiotemporal information for understanding multi-agent dynamics. Additionally, effectively using short-term and long-term observation is crucial for adapting to changes in system dynamics.

